Linear list-approximation for short programs (or the power of a few random bits)

A $c$-short program for a string $x$ is a description of $x$ of length at most $C(x) + c$, where $C(x)$ is the Kolmogorov complexity of $x$. We show that there exists a randomized algorithm that constructs a list of $n$ elements that contains a $O(\log n)$-short program for $x$. We also show a polynomial-time randomized construction that achieves the same list size for $O(\log^2 n)$-short programs. These results beat the lower bounds shown by Bauwens et al. \cite{bmvz:c:shortlist} for deterministic constructions of such lists. We also prove tight lower bounds for the main parameters of our result. The constructions use only $O(\log n)$ ($O(\log^2 n)$ for the polynomial-time result) random bits . Thus using only few random bits it is possible to do tasks that cannot be done by any deterministic algorithm regardless of its running time.

==> macros.tex <==
\usepackage{amsfonts}

\newcommand{\sharpp}{{\rm \#P}}
\newcommand{\sharpsat}{{\rm \#SAT}}
\newcommand{\sat}{{\rm SAT}}
\newcommand{\qbf}{{\rm QBF}}
\newcommand{\parityp}{{\rm \oplus P}}
\newcommand{\up}{{\rm UP}}
\newcommand{\pcp}{{\rm PCP}}
\newcommand{\pcps}{{\rm PCPS}}
\newcommand{\us}{{\rm US}}
\newcommand{\fewnp}{{\rm FewNP}}
\newcommand{\coup}{{\rm coUP}}
\newcommand{\e}{{\rm E}}
\renewcommand{\exp}{{\rm EXP}}
\newcommand{\conexp}{{\rm coNEXP}}
\newcommand{\nat}{{\mathbb N}}
\newcommand{\NE}{{\rm NE}}
\renewcommand{\ne}{{\rm NE}}
\newcommand{\nexp}{{\rm NEXP}}
\newcommand{\p}{{\rm P}}
\newcommand{\pf}{{\rm PF}}
\newcommand{\littlep}{{\rm p}}
\newcommand{\np}{{\rm NP}}
\newcommand{\rp}{{\rm RP}}
\newcommand{\corp}{{\rm coRP}}
\newcommand{\optp}{{\rm OptP}}
\newcommand{\pp}{{\rm PP}}
\newcommand{\bpp}{{\rm BPP}}
\newcommand{\conp}{{\rm coNP}}
\newcommand{\pspace}{{\rm PSPACE}}
\newcommand{\pnplog}{{\p^{\np[\log ]}}}
\newcommand{\pnplogk}{{\p^{\np[\log^k]}}}
\newcommand{\mipgen}{{{\rm MIP}_1(r,p,a,q,\epsilon)}}
\newcommand{\mip}{{\rm MIP}}
\newcommand{\mipone}{{{\rm MIN}_1}}
\newcommand{\sigb}{{\Sigma^{d \cdot \log^3 n}}}
\newcommand{\sigm}{{\Sigma^{d \cdot \log n}}}
\newcommand{\maxnp}{{\rm MAX ~NP}}
\newcommand{\maxsnp}{{\rm MAX ~SNP}}
\newcommand{\MAX}{{\rm MAX}}
\newcommand{\MIN}{{\rm MIN}}
\newcommand{\MAXBF}{{\bf MAX}}
\newcommand{\MINBF}{{\bf MIN}}
\newcommand{\maxfs}[1]{{\MAX ~{\rm F}\Sigma_{#1}}}
\newcommand{\maxfp}[1]{{\MAX ~{\rm F}\Pi_{#1}}}
\newcommand{\minfs}[1]{{\MIN ~{\rm F}\Sigma_{#1}}}
\newcommand{\minfp}[1]{{\MIN ~{\rm F}\Pi_{#1}}}

\newcommand{\minfpp}[1]{{\MIN ~{\rm F^+}\Pi_{#1}}}
\newcommand{\wpminfpp}[1]{{\rm weight(+)}~{\MIN ~{\rm F^+}\Pi_{#1}}}


\newcommand{\opt}{{\rm opt}}

\newcommand{\maxs}[1]{{\MAX ~\Sigma_{#1}}}
\newcommand{\maxp}[1]{{\MAX ~\Pi_{#1}}}
\newcommand{\mins}[1]{{\MIN ~\Sigma_{#1}}}
\newcommand{\minp}[1]{{\MIN ~\Pi_{#1}}}


\newcommand{\wpmaxfs}[1]{{\rm weight(+)}~{\MAX ~{\rm F}\Sigma_{#1}}}
\newcommand{\wpmaxfp}[1]{{\rm weight(+)}~{\MAX ~{\rm F}\Pi_{#1}}}
\newcommand{\wpminfs}[1]{ {\rm weight(+)}~{\MIN ~{\rm F}\Sigma_{#1}}}
\newcommand{\wpminfp}[1]{ {\rm weight(+)}~{\MIN ~{\rm F}\Pi_{#1}}}

\newcommand{\wpmaxs}[1]{ {\rm weight(+)}~{\MAX ~\Sigma_{#1}}}
\newcommand{\wpmaxp}[1]{ {\rm weight(+)}~{\MAX ~\Pi_{#1}}}
\newcommand{\wpmins}[1]{ {\rm weight(+)}~{\MIN ~\Sigma_{#1}}}
\newcommand{\wpminp}[1]{ {\rm weight(+)}~{\MIN ~\Pi_{#1}}}

\newcommand{\wmaxfs}[1]{ {\rm weight}~{\MAX ~{\rm F}\Sigma_{#1}}}
\newcommand{\wmaxfp}[1]{ {\rm weight}~{\MAX ~{\rm F}\Pi_{#1}}}
\newcommand{\wminfs}[1]{ {\rm weight}~{\MIN ~{\rm F}\Sigma_{#1}}}
\newcommand{\wminfp}[1]{ {\rm weight}~{\MIN ~{\rm F}\Pi_{#1}}}

\newcommand{\wmaxs}[1]{ {\rm weight}~{\MAX ~\Sigma_{#1}}}
\newcommand{\wmaxp}[1]{ {\rm weight}~{\MAX ~\Pi_{#1}}}
\newcommand{\wmins}[1]{ {\rm weight}~{\MIN ~\Sigma_{#1}}}
\newcommand{\wminp}[1]{ {\rm weight}~{\MIN ~\Pi_{#1}}}




\newcommand{\maxsizero}{{\MAX ~\Sigma_0}}
\newcommand{\maxsione}{{\MAX ~\Sigma_1}}
\newcommand{\maxsitwo}{{\MAX ~\Sigma_2}}
\newcommand{\minsitwo}{{\MIN ~\Sigma_2}}
\newcommand{\maxpione}{{\MAX ~\Pi_1}}
\newcommand{\maxpitwo}{{\MAX ~\Pi_2}}
\newcommand{\minpitwo}{{\MIN ~\Pi_2}}
\newcommand{\minpione}{{\MIN ~\Pi_1}}
\newcommand{\minsizero}{{\MIN ~\Sigma_0}}
\newcommand{\minsione}{{\MIN ~\Sigma_1}}
\newcommand{\maxfsizero}{{\MAX ~{\rm F}\Sigma_0}}
\newcommand{\wmaxfsione}{{\weight~\MAX ~{\rm F}\Sigma_1}}
\newcommand{\wmaxpfsione}{{\weight(+)~\MAX ~{\rm F}\Sigma_1}}
\newcommand{\wmaxfsitwo}{{\weight~\MAX ~{\rm F}\Sigma_2}}
\newcommand{\wmaxpfsitwo}{{\weight(+)~\MAX ~{\rm F}\Sigma_2}}
\newcommand{\cone}{{\rm CONE}}
\newcommand{\poly}{{\rm poly}}
\newcommand{\ph}{{\rm PH}}
\newcommand{\ch}{{\rm CH}}
\newcommand{\bh}{{\rm BH}}
\newcommand{\few}{{\rm Few}}
%\newcommand{\proof}{{\bf Proof}}
\newcommand{\blob}{\mbox{\rule[-1.5pt]{5pt}{10.5pt}}}
%\newcommand{\ie}{{\mbox{i.e.}}}
\newcommand{\ilog}{{\lfloor \log n \rfloor}}
\newcommand{\lindent}{\qquad}
\def\nottoobig#1{{\hbox{$\left#1\vcenter
to1.111\ht\strutbox{}\right.\n@space$}}}
\newcommand{\condn}{\,\nottoobig{|}\:}
%\ macros from the hypertree paper
\newcommand{\SP}{\mbox{ }}
\newcommand{\comb}[2]{\begin{math}{#1 \choose #2} \end{math}}
\newcommand{\chos}[2]{{#1 \choose #2}}
\newcommand{\prob}{{\rm Prob}}
%\newcommand{\psg}{{\rm pseudo-random generator }}
\newcommand{\sigman}{\Sigma^n}
\newcommand{\sigmal}{\Sigma^l}

%macros for quantum comput.
\newcommand{\CC}{{\bf C}}
\newcommand{\ketz}{|0\rangle}
\newcommand{\ketone}{|1\rangle}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\braket}[2]{\langle#1 | #2\rangle}

%Macros from BlumBaire paper
\newcommand{\propersubset}{\subset}
\newcommand{\la}{\lambda}
\newcommand{\f}{\varphi}
\newcommand{\de}{\delta}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
%\newcommand{\e}{\in}
%\newcommand{\th}{\theta}
\newcommand{\spq}{\stackrel{o}\rightarrow}
\newcommand{\s}{\rightarrow}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\PR}{{\rm PR}}
\newcommand{\FR}{{\rm FR}}
\newcommand{\FPRED}{{\rm FPRED}}
\newcommand{\RPRED}{{\rm RPRED}}
\newcommand{\UU}{{\cal U}}
\newcommand{\OO}{{\cal O}}
\newcommand{\x}{{\bf x}}
%\newcommand{\SP}{\;}
\newcommand{\y}{{\bf y}}
%\newcommand{\rem}{{\bf !!!! REMINDER }\\}
\newcommand{\COM}[2]{{#1 \choose #2}}
\newcommand{\ie}{$\mbox{i.e.}$}
\newcommand{\io}{\mbox{i.o.}}


%Macros from ``On Topological size of p-m-complete degrees

\newcommand{\fj}[1]{$ f_{j}(g^{#1}(w_0)) $}
\newcommand{\fjm}[1]{ f_{j}(g^{#1}(w_0)) }


%Macros from ``Strong Forms of Balanced Immunity''


\renewcommand{\Hat}[1]{ \widehat{#1} }
\renewcommand{\Bar}[1]{\overline{#1}}
\renewcommand{\implies}{\:\Rightarrow\:}
\newcommand{\band}{\bigwedge}
\newcommand{\Band}[3]{(\bigwedge#1\!\!:\,#2\!\!:\,#3)}
\newcommand{\bor}{\bigvee}
\newcommand{\Bor}[3]{(\bigvee#1\!\!:\,#2\!\!:\,#3)}
\newcommand{\Forall}[3]{(\forall #1\!\!:\,#2\!\!:\,#3)}
\newcommand{\Exists}[3]{(\exists #1\!\!:\,#2\!\!:\,#3)}
\newcommand{\Union}[3]{(\bigcup #1\!\!:\,#2\!\!:\,#3)}
% put bounds totally under and use big cup even in text
% WARNING.... in a superscript, this will switch everything to big font! so
% use \cup instead!!!!!!!!!!
%\def\union{\,\displaystyle\bigcup\,}
%\def\inter{\,\displaystyle\bigcap\,}
% the extra brackets should limit the scope of the disp.... we'll see!
\def\union{\,\bigcup\limits}
\def\inter{\,\bigcap\limits\,}
\newcommand{\true}{\mbox{\it true}}
\newcommand{\false}{\mbox{\it false}}
\newcommand{\SUM}[3]{ (\sum #1 \!\! : \, #2 \!\!:\, #3) }
\newcommand{\IFS}{\mbox{\bf if}}
\newcommand{\IF}[1]{ \mbox{\bf if} \, #1 \, \rightarrow \, }
\newcommand{\GC}[2]{ #1 \, \rightarrow \, #2 }
\newlength{\filength}
\settowidth{\filength}{\mbox{\bf f{}i}}
\newsavebox{\gcbox}
\sbox{\gcbox}{\framebox[\filength]{\rule{0ex}{2ex}}}
\newcommand{\BB}[1]{\usebox{\gcbox}\; #1 \, \rightarrow \, }
\newcommand{\FI}{\; \mbox{\bf f{}i}}
\newcommand{\Skip}{ \mbox{\bf skip} }
\newcommand{\DOS}{\mbox{\bf do}}
\newcommand{\DO}[1]{\mbox{\bf do} \, #1 \, \rightarrow \,}
\newcommand{\OD}{\mbox{\bf od}}
\newcommand{\cobegin}{{\bf cobegin}\,}
\renewcommand{\|}{\, //  \,}
\newcommand{\coend}{\,{\bf coend}}
\newcommand{\Set}[1]{ \hbox{\bf\{} #1 \hbox{\bf\}}}
\newcommand{\Bag}[1]{ \{\!| #1  |\!\}}
\newcommand{\hoare}[3]{\{{#1}\}\:{#2}\:\{{#3}\}}
\renewcommand{\wp}[2]{ {\it wp}({#1},{#2})}
\newcommand{\assert}[1]{\!\{#1\}}
\newcommand{\atom}[1]{\langle\,{#1}\,\rangle}
\newcommand{\lbl}[1]{{#1 \!:\;\,}}
\newcommand{\pre}[1]{ {\it pre}({#1})}
\newcommand{\post}[1]{ {\it post}({#1}) }
\newcommand{\NI}[2]{ {\it NI}({#1},{#2}) }
\newcommand{\equi}[3]{ {  {\rm E}_{#1}^{#2}({#3}) }    }
\newcommand{\red}[3]{ {  {\rm R}_{#1}^{#2}({#3}) }    }
\newcommand{\sparse}{{{\rm SPARSE}}}
\newcommand{\tally}{{{\rm TALLY}}}
\newcommand{\inferfrom}[2]{\begin{array}[t]{c}\displaystyle
   \frac{#1}{#2}\end{array}}
% The followiing are the \newcommands from mybim.tex of Marius Zimand
%\newcommand{\comb}[2]{\begin{math}{#1 \choose #2} \end{math}}
\newcommand{\lcard}{\frac{| (L(M^A) \cap T(A)) ^{\leq n}|}{| L(M^A) 
^{\leq n}|}}
\newcommand{\nt}{{\rm NT}}
\newcommand{\NT}{{\rm NT}}
\newcommand{\nnt}{{\rm NNT}}
\newcommand{\npa}{\mbox{$\np^A$}}
\newcommand{\conpa}{\mbox{$\conp^A$}}
\newcommand{\upa}{\mbox{$\up^A$}}
\newcommand{\parityoptp}{{\rm \oplus{}OptP}}
%\newcommand{\optp}{{\rm OptP}}
\newcommand{\diffp}{{\rm D^P}}
%\newcommand{\pp}{{\rm PP}}
%\newcommand{\bpp}{{\rm BPP}}
%\newcommand{\cor}{{\rm coR}}
\newcommand{\npc}{$\np$-com\-plete}
\newcommand{\qedblob}{\mbox{\rule[-1.5pt]{5pt}{10.5pt}}}
\def\literalqed{{\ \nolinebreak\hfill\mbox{\qedblob\quad}}}
\def\qedcareful{\literalqed}
\def\qed{\literalqed}
\def\trueloveqed{{\ \nolinebreak\hfill\mbox{\boldmath
\Huge$ \Box$}\nolinebreak\mbox{$\!\!\!\!\!\!
{}^{\normalsize\heartsuit}$}}}
\newcommand{\bigo}{\mbox{$\cal O$}}
%\newcommand{\condition}{\,\nottoobig{|}\:}
\newcommand{\condition}{{|}}
\newcommand{\sigmastar}{\mbox{$\Sigma^\ast$}}
\newcommand{\sigmak}{{\Sigma_k^p}}
\newcommand{\pik}{{\Pi_k^p}}
%\newcommand{\parityp}{{\rm \oplus P}}








%\newcommand{\up}{{\rm UP}}
%\newcommand{\us}{{\rm US}}
%\newcommand{\fewnp}{{\rm FewNP}}
\newcommand{\fewp}{{\rm FewP}}
%\newcommand{\coup}{{\rm coUP}}
%\newcommand{\e}{{\rm E}}
\renewcommand{\exp}{{\rm EXP}}
%\newcommand{\NE}{{\rm NE}}
\renewcommand{\ne}{{\rm NE}}
%\newcommand{\nexp}{{\rm NEXP}}
\newcommand{\sigmakx}{{\Sigma_{k+1}^p}}
\newcommand{\pikx}{{\Pi_{k+1}^p}}
\newcommand{\invb}{INVBOUND^A}
\newcommand{\invbG}{INVBOUND^G}
\newcommand{\alf}{\{0, 1\}^{l(n)}}

%Macros from Martin-Lof tests

\newcommand{\kc}{\mbox{Kolmogorov complexity}}
\newcommand{\ml}{\mbox{Martin-L\"{o}f}}
\newcommand{\re}{\mbox{\mbox{r.e.}}}


%Macros for hastad.tex
\newcommand{\cro}{{C|_{\rho}}}
\newcommand{\cirr}{{C|_{\rho_{1} \rho_{2}}}}
\newcommand{\dr}{{D|_{\rho}}}
\newcommand{\drr}{{D|_{\rho_1 \rho_2}}}
\newcommand{\AO}{\mbox{AND-of-ORs}}
\newcommand{\OA}{\mbox{OR-of-ANDs}}
\newcommand{\dfr}{\Delta(f|_{\rho})}
\newcommand{\sAO}{{s-\mbox{AND-of-ORs circuit } }}
\newcommand{\tOA}{t-\mbox{OR-of-ANDs circuit } }
\newcommand{\tAO}{{t-\mbox{AND-of-ORs circuit } }}
\newcommand{\sOA}{s-\mbox{OR-of-ANDs circuit } }

\newcommand{\gr}{{G_{1}|_{\rho}}}
\newcommand{\grr}{{G_{1}|_{\rho_1 \rho_2}}}
\newcommand{\Fr}{{F|_{\rho}}}
\newcommand{\Frr}{{F|_{\rho_1 \rho_2}}}
\newcommand{\myc}{{min^{Y}(C|_{\rho})}}
\newcommand{\mysc}{{min^{Y, \sigma}(C|_{\rho})}}
\newcommand{\myscc}{{min^{Y, \sigma}(C|_{\rho_1 \rho_2})}}


%\newcommand{\SP}{\mbox{ }}
%\newcommand{\ie}{$\mbox{i.e.}$}
%\newtheorem{Theorem}{Theorem}
%\newtheorem{Lemma}{Lemma}
%\newenvironment{proof}{\Proof}{\qed}

%MY-EXPERIMENT
%\newcommand{\myspacing}{\let\CS=
%\currsize\renewcommand{\baselinestretch}{2}\CS}     

%END MY EXPERIMENT

\newcommand{\singlespacing}{\let\CS=
\@currsize\renewcommand{\baselinestretch}{1}\tiny\CS}
\newcommand{\singlespacingplus}{\let\CS=
\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}
\newcommand{\doublespacing}{\let\CS=
\@currsize\renewcommand{\baselinestretch}{1.75}\tiny\CS}
\newcommand{\draftspacing}{\let\CS=
\@currsize\renewcommand{\baselinestretch}{2.0}\tiny\CS}
\newcommand{\normalspacing}{\singlespacing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%other popular characters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\sstar{\Sigma^{*}}
\def\sinf{\Sigma^{\infty}}
\def\ssinf{\Sigma^{\infty}}
\def\zeroone{\{0,1\}}
\def\zo{\{0,1\}}
\def\ORD{\mbox{{\rm ord}}}
\def\square{\rlap{$\sqcup$}$\sqcap$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%logical sumbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\AND{\wedge}
\def\OR{\vee}
\def\oper{\circ}
\def\mapping{\rightarrow}
\def\implies{\rightarrow}

\def\L{\langle}
\def\R{\rangle}

\def\HYP{\hbox{-}}
\def\IFF{\leftrightarrow}
\def\Ldef{\buildrel \rm def \over \leftrightarrow}
\def\Edef{\buildrel \rm def \over =}
\def\almostall{\hbox{\rlap{$_{\thinspace\forall}$}{$^{^\infty}$}}}
\def\infoften{\hbox{\rlap{$_{\thinspace\exists}$}{$^{^\infty}$}}}
\def\NUM{{\bf N}}
\newcommand{\Z}{\mathbb{Z}}
\def\z{{\bf Z}}
%\input{global.mac}
%\input{local.mac}

\def\calI{{\cal I}}
\def\calF{{\cal F}}
\newcommand{\bara}[1]{{\overline #1}}


%%%%%%%%%%%%%%%%%%%%%%% pmeas.tex%%%%%%%%%%%%%%%%%%%%

\def\HYP{\hbox{-}}
\def\IFF{\leftrightarrow}
\def\Ldef{\buildrel \rm def \over \leftrightarrow}
\def\Edef{\buildrel \rm def \over =}
\def\almostall{\hbox{\rlap{$_{\thinspace\forall}$}{$^{^\infty}$}}}
\def\infoften{\hbox{\rlap{$_{\thinspace\exists}$}{$^{^\infty}$}}}
\def\NUM{{\bf N}}
\def\REAL{{\bf R}}


\def\calC{{\cal C}}

\newcommand{\fp}{{\rm FP}}

\def\ssl{\Sigma^{S(L)}}
\def\sl{\Sigma^{L}}



%%%%%%%%%%%%%%% from aczero.tex%%%%%%%%%%%%%%%
\newcommand{\acc}{{\rm ACC}}
%\newcommand{\nc}{{\rm NC}}
\newcommand{\ncone}{{\nc^1}}
\newcommand{\ac}{{\rm AC}}
\newcommand{\acz}{{\ac^0}}
\newcommand{\ptopp}{{\p^{\pp}}}
%\newcommand{\mipgen}{{{\rm MIP}_1(r(n),p(n),a(n),q(n),\epsilon(n))}}
%\newcommand{\NUM}{{\bf N}}
%\newcommand{\REAL}{{\bf R}}
%\newcommand{\kc}{\mbox{Kolmogorov complexity}}
%\newcommand{\ml}{\mbox{Martin-L\"{o}f}}


%%%%%%%%%%%%%% from randprim.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ildn}{{\lfloor (\ln 2) n\rfloor}}
\def\calA{{\cal A}}
\def\calC{{\cal C}}
\def\calI{{\cal I}}
\def\calF{{\cal F}}
\def\calR{{\cal R}}
\def\calS{{\cal S}}
%\newcommand{\bara}[1]{{\overline #1}}

\newcommand{\probxr}{{Prob_{x, R}}}
\newcommand{\probyr}{{Prob_{y, R}}} 


\def\sstar{\Sigma^{*}}
\newcommand{\sn}{\Sigma^{n}}
\newcommand{\stwon}{\Sigma^{2n}}
%\def\sigmatwon{\Sigma^{2n}}
%\def\sigmaen{\Sigma^{8n}}
%\def\sigmasn{\Sigma^{16n}}




% mathematical symbols from amstex

%\input amssym.def
%\input amssym.tex             % This works, too.
%\newsymbol\subseteqq 136A
%\newsymbol\supseteqq 136B
%\newsymbol\nsubseteqq 2322
%\newsymbol\nsupseteqq 2323
%\newsymbol\subsetneqq 2324
%\newsymbol\supsetneqq 2325










